TATi-Thermodynamic Analytics ToolkIt: TensorFlow-based software for posterior sampling in machine learning applications

With the advent of GPU-assisted hardware and maturing high-efficiency software platforms such as TensorFlow and PyTorch, Bayesian posterior sampling for neural networks becomes plausible. In this article we discuss Bayesian parametrization in machine learning based on Markov Chain Monte Carlo methods, specifically discretized stochastic differential equations such as Langevin dynamics and extended system methods in which an ensemble of walkers is employed to enhance sampling. We provide a glimpse of the potential of the sampling-intensive approach by studying (and visualizing) the loss landscape of a neural network applied to the MNIST data set. Moreover, we investigate how the sampling efficiency itself can be significantly enhanced through an ensemble quasi-Newton preconditioning method. This article accompanies the release of a new TensorFlow software package, the Thermodynamic Analytics ToolkIt, which is used in the computational experiments.

==> figures/09_Benchmarking_MNIST/runtimes_per_dof-sampler-relative-comparison.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Pipelines comparison - dataset and network size}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/09_Benchmarking_MNIST/data}\fi%

%special column names
\ifdefined\myxcolumnname\empty\else\def\myxcolumnname{hidden_dimension}\fi%
\ifdefined\myycolumnname\empty\else\def\myycolumnname{time_per_nth_step}\fi%
%parameters
\ifdefined\mysampler\empty\else\def\mysampler{BAOAB}\fi% %BAOAB, GeometricLangevinAlgorithm_1stOrder, GeometricLangevinAlgorithm_2ndOrder, StochasticGradientLangevinDynamics
\ifdefined\mysamplername\empty\else\def\mysamplername{BAOAB}\fi% %BAOAB, GLA1, GLA2, SGLD
\ifdefined\myinmemorypipeline\empty\else\def\myinmemorypipeline{0}\fi% %0, 1
\ifdefined\myhiddendimension\empty\else\def\mydimension{5000}\fi% %500,1600,5000,16000
\ifdefined\mybatchsize\empty\else\def\mybatchsize{100}\fi% %100, 1000, 10000


% parse tables
%SGLD
\pgfplotstableread[columns={\myxcolumnname,avg_\myycolumnname,var_\myycolumnname}, col sep=comma]{\mypath/Pipelines_comparison_-_dataset_and_network_size/runtimes_per_step-batch_size_\mybatchsize-dimension_\mydimension-in_memory_pipeline_\myinmemorypipeline-sampler_StochasticGradientLangevinDynamics.csv}\mysgldtable


% GLA1
\pgfplotstableread[columns={\myxcolumnname,avg_\myycolumnname,var_\myycolumnname}, col sep=comma]{\mypath/Pipelines_comparison_-_dataset_and_network_size/runtimes_per_step-batch_size_\mybatchsize-dimension_\mydimension-in_memory_pipeline_\myinmemorypipeline-sampler_GeometricLangevinAlgorithm_1stOrder.csv}\myglaonetable

% GLA2
\pgfplotstableread[columns={\myxcolumnname,avg_\myycolumnname,var_\myycolumnname}, col sep=comma]{\mypath/Pipelines_comparison_-_dataset_and_network_size/runtimes_per_step-batch_size_\mybatchsize-dimension_\mydimension-in_memory_pipeline_\myinmemorypipeline-sampler_GeometricLangevinAlgorithm_2ndOrder.csv}\myglatwotable

% BAOAB
\pgfplotstableread[columns={\myxcolumnname,avg_\myycolumnname,var_\myycolumnname}, col sep=comma]{\mypath/Pipelines_comparison_-_dataset_and_network_size/runtimes_per_step-batch_size_\mybatchsize-dimension_\mydimension-in_memory_pipeline_\myinmemorypipeline-sampler_BAOAB.csv}\mybaoabtable

% GD-rand
\pgfplotstableread[columns={\myxcolumnname,avg_\myycolumnname,var_\myycolumnname}, col sep=comma]{\mypath/Pipelines_comparison_-_opt_rand_-_dataset_and_network_size/runtimes_per_step-batch_size_\mybatchsize-dimension_\mydimension-in_memory_pipeline_\myinmemorypipeline.csv}\mygdrandtable

% GD
\pgfplotstableread[columns={\myxcolumnname,avg_\myycolumnname,var_\myycolumnname}, col sep=comma]{\mypath/Pipelines_comparison_-_opt_-_dataset_and_network_size/runtimes_per_step-batch_size_\mybatchsize-dimension_\mydimension-in_memory_pipeline_\myinmemorypipeline.csv}\mygdtable

\pgfplotstableset{
	create on use/BAOAB_runtime/.style={create col/copy column from table={\mybaoabtable}{avg_\myycolumnname}},
	create on use/GD_runtime/.style={create col/copy column from table={\mygdtable}{avg_\myycolumnname}},
	create on use/GLA1_runtime/.style={create col/copy column from table={\myglaonetable}{avg_\myycolumnname}},
	create on use/GLA2_runtime/.style={create col/copy column from table={\myglatwotable}{avg_\myycolumnname}},
	create on use/GDrand_runtime/.style={create col/copy column from table={\mygdrandtable}{avg_\myycolumnname}},
	create on use/SGLD_runtime/.style={create col/copy column from table={\mysgldtable}{avg_\myycolumnname}},
	create on use/\myxcolumnname/.style={create col/copy column from table={\mysgldtable}{\myxcolumnname}},
	create on use/dof/.style={create col/expr={(784+10)*\thisrow{\myxcolumnname}+\thisrow{\myxcolumnname}+10}},
}

\pgfplotstablegetrowsof\mybaoabtable%

\pgfplotstablenew[columns={\myxcolumnname,BAOAB_runtime,GD_runtime,GDrand_runtime,GLA1_runtime,GLA2_runtime,SGLD_runtime}]{\pgfmathresult}\mycomparisontable

\begin{tikzpicture}[]
\begin{semilogxaxis}[
	width=7cm,height=6cm,
	%title style={align=left},
	%title = {\emph{\myexperimentname}:\\ \expandafter\escapeus\expandafter{in_memory_pipeline}=\pgfmathprintnumber{\myinmemorypipeline}, \expandafter\escapeus\expandafter{dimension}=\pgfmathprintnumber{\mydimension}, \expandafter\escapeus\expandafter{batch_size}=\pgfmathprintnumber{\mybatchsize}},
	xlabel = {Degrees of freedom of network},
	ylabel = {Relative runtime w.r.t. GD},
	%xtick={1600,16000,500,5000},
%	ymin=0.02,ymax=0.2,
	%log ticks with fixed point,
	legend pos=outer north east,
	%cycle list name=exotic,
	cycle multi list={
		{mark=o,red},{mark=star,blue},{mark=|,brown},{mark=x,green},{mark=square,black},{mark=otimes,gray}
	},
	grid=major,
%	each nth point=1,
]
\pgfplotsinvokeforeach{SGLD,GLA1,GLA2,BAOAB,GDrand,GD}{%
\addplot+[thick,error bars/.cd, y dir=both, y explicit] table[x=dof,y expr ={\thisrow{#1_runtime}/\thisrow{GD_runtime}}]\mycomparisontable;
\addlegendentry{#1}
}
\end{semilogxaxis}
\end{tikzpicture}


==> figures/09_Benchmarking_MNIST/step_time_per_nth_step.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Pipelines comparison - dataset and network size}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/09_Benchmarking_MNIST/data/Pipelines_comparison_-_dataset_and_network_size}\fi%

%special column names
\ifdefined\myxcolumnname\empty\else\def\myxcolumnname{dimension}\fi%
\ifdefined\myycolumnname\empty\else\def\myycolumnname{avg_time_per_nth_step}\fi%
%parameters
\ifdefined\myhiddendimension\empty\else\def\myhiddendimension{1000}\fi% %0, 10, 100, 1000
\ifdefined\mybatchsize\empty\else\def\mybatchsize{100}\fi% %100, 1000, 10000
\ifdefined\mydimension\empty\else\def\mydimension{5000}\fi% %500,1600,5000,16000
\ifdefined\mypipeline\empty\else\def\mypipeline{0}\fi% %0, 1
\ifdefined\mysampler\empty\else\def\mysampler{BAOAB}\fi% %StochasticGradientLangevinDynamics, GeometricLangevinAlgorithm_1stOrder, GeometricLangevinAlgorithm_2ndOrder, BAOAB
\ifdefined\myseed\empty\else\def\myseed{426}\fi% %426, 427, 428

\begin{tikzpicture}[]
\begin{semilogyaxis}[
	title style={align=left},
	title = {\emph{\myexperimentname}:\\ \expandafter\escapeus\expandafter{hidden_dimension}=\pgfmathprintnumber{\myhiddendimension}, \expandafter\escapeus\expandafter{dimension}=\pgfmathprintnumber{\mydimension},  \expandafter\escapeus\expandafter{batch_size}=\pgfmathprintnumber{\mybatchsize}},
	xlabel={step},
	ylabel={time per 10 steps [s]},
	ymin=0.075,ymax=3,
	log ticks with fixed point,
	legend pos=outer north east,
	grid=major,
	legend pos=north east,
%	cycle list name=exotic,
	filter discard warning=false,
%	each nth point=\myeverynth,
]
\addlegendimage{empty legend}
\addlegendentry{\escapeus{sampler}}
\foreach \mysampler\mysamplername in {StochasticGradientLangevinDynamics/SGLD, GeometricLangevinAlgorithm_1stOrder/GLA1, GeometricLangevinAlgorithm_2ndOrder/GLA2, BAOAB/BAOAB}{%
\addplot+[thick, no marks] table[x expr={\thisrow{step}-1000},y=time_per_nth_step,col sep=comma]{\mypath/run-batch_size_\mybatchsize-dimension_\mydimension-hidden_dimension_\myhiddendimension-in_memory_pipeline_\mypipeline-sampler_\mysampler-seed_\myseed.csv};
\addlegendentryexpanded{\mysamplername}
}%
\end{semilogyaxis}
\end{tikzpicture}



==> figures/10_OrderOfDecay_TwoClusters/order_of_decay-slope_fit-all_samplers-kinetic.tex <==
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/10_OrderOfDecay_TwoClusters/data/}\fi%

% parameter
\ifdefined\mysamplername\empty\else\def\mysampler{StochasticGradientLangevinDynamics}\fi%
\ifdefined\mysamplername\empty\else\def\mysamplername{SGLD}\fi%
\ifdefined\mybeta\empty\else\def\mybeta{10}\fi%
\ifdefined\mygamma\empty\else\def\mygamma{10}\fi%

\def\mydof{3}%
\def\myasymptoticloss{0.2349601251}%

\ifdefined\mycolumn\empty\else\def\mycolumn{kinetic_energy}\fi%

% samplers

% SGLD
\pgfplotstableread[columns={step_width,average_\mycolumnname}, col sep=comma]{\mypath/Order_of_decay_-_SGLD/average_degrees_of_freedom-friction_constant_\mygamma-inverse_temperature_\mybeta-sampler_StochasticGradientLangevinDynamics.csv}\mysgldtable
% GLA1
\pgfplotstableread[columns={step_width,average_\mycolumnname}, col sep=comma]{\mypath/Order_of_decay_-_GLA1/average_degrees_of_freedom-friction_constant_\mygamma-inverse_temperature_\mybeta-sampler_GeometricLangevinAlgorithm_1stOrder.csv}\myglaonetable
% GLA2
\pgfplotstableread[columns={step_width,average_\mycolumnname}, col sep=comma]{\mypath/Order_of_decay_-_GLA2/average_degrees_of_freedom-friction_constant_\mygamma-inverse_temperature_\mybeta-sampler_GeometricLangevinAlgorithm_2ndOrder.csv}\myglatwotable
% BAOAB
\pgfplotstableread[columns={step_width,average_\mycolumnname}, col sep=comma]{\mypath/Order_of_decay_-_BAOAB/average_degrees_of_freedom-friction_constant_\mygamma-inverse_temperature_\mybeta-sampler_BAOAB.csv}\mybaoabtable

\pgfplotstablegetrowsof\mysgldtable%

\pgfplotstableset{
	create on use/virials_error/.style={create col/expr={abs(\mydof/2-\thisrow{avg_average_virials}*\mybeta)}},
	create on use/kinetic_energy_error/.style={create col/expr={abs(\mydof/2-\thisrow{avg_average_kinetic_energy}*\mybeta)}},
	create on use/potential_error/.style={create col/expr={abs(\myasymptoticloss-\thisrow{avg_ensemble_average_loss})}},
}

% \pgfplotstablecreatecol[
% 	create on use/error/.style={create col/expr={abs(\mydof/2-\thisrow{avg_average_\mycolumnname}*1e1)}},
% ]{error}{\myglafirsttable}
%\pgfplotstablecreatecol[linear regression]{linear_regression}{\myglafirsttable}
%\xdef\slopeGLAfirst{\pgfplotstableregressiona}

% \pgfplotstablecreatecol{error}{\myglasecondtable}
%\pgfplotstablecreatecol[linear regression]{error}{\myglasecondtable}
%\xdef\slopeGLAsecond{\pgfplotstableregressiona}

\begin{tikzpicture}[]
% \node (a)  {\pgfplotstabletypeset[columns={step_width}]\myglafirsttable};
\begin{loglogaxis}[
	thick,
%	title={Order of decay - all samplers: \expandafter\spaceus\expandafter{\mycolumn}, $\beta = \pgfmathprintnumber{\mybeta}$, $\gamma = \pgfmathprintnumber{\mygamma}$},
	xlabel = {step width},
	ylabel = {$\Bigl | \tfrac {N_{\text{DOF}}} 2 - E^{\text{avg}}_{\text{kin}}
\cdot \beta \Bigr |$},
	grid=major,
	legend style={at={(1,1.275)}},
%	legend pos=outer north east,
	legend columns=2,
%	xtick={0.25,0.125,0.0625,0.03125,0.015625},
]
% % SGLD/Euler-Maruyama
% \addplot+[red,solid, mark=o] table[x=step_width,y=\mycolumn_error]\mysgldtable;
% \addlegendentry{}
% 
% \addplot+[red, dashed,no marks] table[x=step_width, y={create col/linear regression={x=step_width,y=\mycolumn_error, variance list={1,1,1,1,100}}}]\mysgldtable;
% \xdef\slopesgld{\pgfplotstableregressiona}
% \addlegendentry{slope SGLD: \pgfmathprintnumber{\slopesgld}}

% GLA1
\addplot+[blue,solid, mark=o] table[x=step_width,y=\mycolumn_error]\myglaonetable;
\addlegendentry{}

\addplot+[blue, dashed,no marks] table[x=step_width, y={create col/linear regression={x=step_width,y=\mycolumn_error, variance list={1,1,1,1,100}}}]\myglaonetable;
\xdef\slopeglaone{\pgfplotstableregressiona}
\addlegendentry{slope GLA1: \pgfmathprintnumber{\slopeglaone}}

% GLA2
\addplot+[brown,solid, mark=o] table[x=step_width,y=\mycolumn_error]\myglatwotable;
\addlegendentry{}

\addplot+[brown, dashed,no marks] table[x=step_width, y={create col/linear regression={x=step_width,y=\mycolumn_error, variance list={1,1,1,1,100}}}]\myglatwotable;
\xdef\slopeglatwo{\pgfplotstableregressiona}
\addlegendentry{slope GLA2: \pgfmathprintnumber{\slopeglatwo}}

% BAOAB
\addplot+[black,solid, mark=o] table[x=step_width,y=\mycolumn_error]\mybaoabtable;
\addlegendentry{}

\addplot+[black, dashed,no marks] table[x=step_width, y={create col/linear regression={x=step_width,y=\mycolumn_error, variance list={1,1,1,1,100}}}]\mybaoabtable;
\xdef\slopebaoab{\pgfplotstableregressiona}
\addlegendentry{slope BAOAB: \pgfmathprintnumber{\slopebaoab}}
\end{loglogaxis}
\end{tikzpicture}

==> figures/13_EnsemblePreconditioning_MNIST/autocorrelation-individual_time-number_walkers.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Sampling MNIST - EQN TATi}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/13_EnsemblePreconditioning_MNIST/data/Sampling_MNIST_-_EQN_TATi}\fi%

%special column names
\ifdefined\myxcolumnname\empty\else\def\myxcolumnname{weight}\fi%
\ifdefined\myycolumnname\empty\else\def\myycolumnname{tau}\fi%
%parameters
\ifdefined\mynumberwalkers\empty\else\def\mynumberwalkers{8}\fi% %8
\ifdefined\mybatchsize\empty\else\def\mybatchsize{550}\fi% %8

\begin{tikzpicture}[]
\begin{axis}[
	width=8.5cm,height=7.25cm,
	%title style={align=left},
	%title = {\emph{\myexperimentname}: comparing walkers},
	xlabel = {Coordinate index},
	ylabel = {Integated Autocorrelation Time $\tau$},
	legend pos=north east,
	grid=major,
%	each nth point=1,
]
\addlegendimage{empty legend}
\addlegendentry{$\eta$}
\foreach \myeta in {0,1,2.5,10}{%
\addplot+[
	error bars/.cd,
        y dir=both,
        y explicit
] table[x=\myxcolumnname,y=avg_\myycolumnname, y error expr={sqrt(abs(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2))}, col sep=comma]{\mypath/autocorrelation-individual_time-batch_size_\mybatchsize-covariance_blending_\myeta.csv};
\addlegendentryexpanded{\myeta}
}
\end{axis}
\end{tikzpicture}


==> figures/13_EnsemblePreconditioning_MNIST/step-loss.tex <==
\ifdefined\myexperiment\empty\else\def\myexperiment{Sampling_MNIST}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/13_EnsemblePreconditioning_MNIST/data/\myexperiment}\fi% %

% parameter
\ifdefined\mybeta\empty\else\def\mybeta{10}\fi%
\ifdefined\mydeltat\empty\else\def\mydeltat{0_125}\fi%
\ifdefined\mygamma\empty\else\def\mygamma{10}\fi%

\ifdefined\mycolumnname\empty\else\def\mycolumnname{loss}\fi%\StrSubstitute

\ifdefined\mydof\empty\else\def\mydof{7850}\fi% 784*10+10 (weights + biases)

\begin{tikzpicture}[]
\begin{axis}[
	width=8.5cm,height=7.25cm,
	%title style={align=left},
	%title={\expandafter\spaceus\expandafter{\myexperiment}: \\ $\gamma=\pgfmathprintnumber{\mygamma}$, $\beta=\expandafter\dotus\expandafter{\mybeta}$, $\Delta t=\expandafter\dotus\expandafter{\mydeltat}$}, 
	grid=major,
	xlabel={Step},
	ylabel={Loss},
	legend pos=south east,
	each nth point=10,
%	restrict y to domain*={50:60},
%	restrict x to domain={0:2e5},
	cycle multi list={
		red,blue, black
	},
]
\addlegendimage{empty legend}
\addlegendentry{seed}
\foreach \myseed in {426,427,428}{%
% loss
\addplot+[thick,no marks] table[x=step,y=\mycolumnname, col sep=comma]{\mypath/run-batch_size_550-run_seed_\myseed.csv};
\addlegendentryexpanded{\myseed}
}%
\end{axis}
\end{tikzpicture}

==> figures/15_Asymptotic_Kinetic_Error/Flat_potential/average_kinetic_error-step-loglog-fit.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Flat potential}\fi%
\ifdefined\mypath\empty\else\def\mypath{/nosave/heber/ExperimentationGrounds/ThermodynamicAnalyticsToolkit/15_Asymptotic_Kinetic_Error/measure/Flat_potential/}\fi%

%special column names
\ifdefined\myxcolumnname\empty\else\def\myxcolumnname{step}\fi%
\ifdefined\myycolumnname\empty\else\def\myycolumnname{average_momentum}\fi%
%parameters
\ifdefined\mystepwidth\empty\else\def\mystepwidth{0_25}\fi% %0.015625, 0.03125, 0.0625, 0.125, 0.25
%\ifdefined\mystepwidthdot\empty\else\def\mystepwidthdot{0.125}\fi% %0.015625, 0.03125, 0.0625, 0.125, 0.25
\ifdefined\myseed\empty\else\def\myseed{426}\fi% %426,427,...,435
%\ifdefined\mygamma\empty\else\def\mygamma{100}\fi% %0.01, 0.1, 1, 10, 100
%\def\mygammadot{\expandafter\dotus\expandafter{\mygamma}}%

\begin{tikzpicture}[]
\begin{loglogaxis}[
	width=8.5cm,height=7.25cm,
	%title style={align=left},
	%title = {\emph{\myexperimentname}:\\ \expandafter\escapeus\expandafter{step_width}=\pgfmathprintnumber{\mystepwidthdot}},
	xlabel = {Step},
	ylabel = {Kinetic energy error $|\hat{\varphi}_N - E_{\mu}[\varphi]|$},
	legend pos=south west,
	grid=major,
	ymin=1e-6,ymax=100,
%	each nth point=1,
	cycle multi list={
		solid, dashed\nextlist
		black,red,blue,brown,green
	},
	legend columns=1,
]
\addlegendimage{empty legend}
\addlegendentry{$\gamma$}
\foreach \mygamma/\mygammadot in {0_01/0.01,0_1/0.1,1/1,10/10,100/100}{%
\addplot+[thick,no marks] table[x=\myxcolumnname,y=average_kinetic_error, col sep=comma]{\mypath/output-gamma_\mygamma-seed_\myseed-step_width_\mystepwidth.csv};
\expandafter\addlegendentry\expandafter{\mygammadot}
}
\foreach \mygamma/\mygammadot in {0_01/0.01,0_1/0.1,1/1,10/10,100/100}{%
\pgfplotstableread[col sep=comma]{\mypath/fit-gamma_\mygamma-seed_\myseed-step_width_\mystepwidth.csv}\myfittable
\pgfplotstablegetrowsof\myfittable%
\pgfmathparse{\pgfplotsretval-1}%
\xdef\mylastrow{\pgfmathresult}%
\pgfplotstablegetelem{\mylastrow}{offset}\of\myfittable%
\xdef\myoptczero{\pgfplotsretval}%
\pgfplotstablegetelem{\mylastrow}{slope}\of\myfittable%
\xdef\myoptcone{\pgfplotsretval}%

\addplot+[domain={1:1e6}, samples=100] {exp(\myoptcone*ln(x)+ \myoptczero)};
%\addlegendentryexpanded{\myoptcone, \myoptczero}
}%
\end{loglogaxis}
\end{tikzpicture}


==> figures/15_Asymptotic_Kinetic_Error/Flat_potential/step_width-asymptotic_error-averaged-slope_fit.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Flat potential}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/15_Asymptotic_Kinetic_Error/data/Flat_potential}\fi%

\def\myycolumnname{final_mean_value}%

\begin{tikzpicture}[]
\begin{loglogaxis}[
	width=7cm,height=6cm,
	%title={Order of convergence},
	xlabel = {Step width},
	ylabel = {Kinetic energy error $E[|\hat{\varphi}_N - E_{\mu}[\varphi]|]$},
	grid=major,
%	legend style={at={(1,1.4)}},
	legend pos=outer north east,
	legend columns=1,
	xtick={0.25,0.125,0.0625,0.03125,0.015625},
	log ticks with fixed point,
	cycle list={
		{blue},{mark=o,blue},
		{red},{mark=square,red},
		{brown},{mark=otimes, brown},
		{black},{mark=star,black},
		{green},{mark=diamond,green}
	},
]
\addlegendimage{empty legend}
\addlegendentry{$\gamma$}
\foreach \mygamma/\mygammadot in {0_01/0.01,0_1/0.1,1/1,10/10,100/100}{%
\pgfplotstableread[columns={step_width,avg_\myycolumnname}, col sep=comma]{\mypath/estimated-gamma_\mygammadot.csv}\mybaoabtable

\addplot+[thick,dotted] table[x=step_width, y={create col/linear regression={x=step_width,y=avg_\myycolumnname, variance list={100,10,1,1,1}}}]\mybaoabtable;
\xdef\slopeglaone{\pgfplotstableregressiona}
\addlegendentryexpanded{slope: \pgfmathprintnumber[fixed,precision=2]{\slopeglaone}}

\addplot+[thick,
	error bars/.cd,
        y dir=both,
        y explicit
] table[x=step_width,y=avg_\myycolumnname, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^ 2)}, col sep=comma]{\mypath/estimated-gamma_\mygammadot.csv};
\expandafter\addlegendentry\expandafter{\mygammadot}

% \addplot+[thick,error bars/.cd, y dir=both, y explicit] table[x=step_width,y expr={abs(0.05-\thisrow{avg_\myycolumnname})/0.05}, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)/0.05}, col sep=comma]{\mypath/estimated-gamma_\mygammadot.csv};
% \expandafter\addlegendentry\expandafter{\mygammadot}
}%
\end{loglogaxis}
\end{tikzpicture}

==> figures/15_Asymptotic_Kinetic_Error/Flat_potential/step_width-asymptotic_error-averaged.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Flat potential}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/15_Asymptotic_Kinetic_Error/data/Flat_potential}\fi%

\def\myycolumnname{final_mean_value}%

\begin{tikzpicture}[]
\begin{loglogaxis}[
	width=7cm,height=6cm,
	%title={Order of convergence},
	xlabel = {Step width},
	ylabel = {Kinetic energy error $E[|\hat{\varphi}_N - E_{\mu}[\varphi]|]$},
	grid=major,
%	legend style={at={(1,1.4)}},
	legend pos=outer north east,
	legend columns=1,
	xtick={0.25,0.125,0.0625,0.03125,0.015625},
	log ticks with fixed point,
	cycle list={
		{mark=o,blue},{mark=square,red},{mark=otimes, brown},{mark=star,black},{mark=diamond,green}
	},
]
\addlegendimage{empty legend}
\addlegendentry{$\gamma$}
\foreach \mygamma/\mygammadot in {0_01/0.01,0_1/0.1,1/1,10/10,100/100}{%
\addplot+[thick,
	error bars/.cd,
        y dir=both,
        y explicit
] table[x=step_width,y=avg_\myycolumnname, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^ 2)}, col sep=comma]{\mypath/estimated-gamma_\mygammadot.csv};
\expandafter\addlegendentry\expandafter{\mygammadot}
}%
\end{loglogaxis}
\end{tikzpicture}

==> figures/15_Asymptotic_Kinetic_Error/Flat_potential/step_width-asymptotic_error-averaged_then_fitted-slope_fit.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Flat potential}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/15_Asymptotic_Kinetic_Error/data/Flat_potential}\fi%

\def\myycolumnname{final_mean_value}%

\begin{tikzpicture}[]
\begin{loglogaxis}[
	width=7cm,height=6cm,
	%title={Order of convergence},
	xlabel = {Step width},
	ylabel = {Kinetic energy error $E[|\hat{\varphi}_N - E_{\mu}[\varphi]|]$},
	grid=major,
%	legend style={at={(1,1.4)}},
	legend pos=outer north east,
	legend columns=1,
	xtick={0.25,0.125,0.0625,0.03125,0.015625},
	log ticks with fixed point,
	cycle list={
		{blue},{mark=o,blue},
		{red},{mark=square,red},
		{brown},{mark=otimes, brown},
		{black},{mark=star,black},
		{green},{mark=diamond,green}
	},
]
\addlegendimage{empty legend}
\addlegendentry{$\gamma$}
\foreach \mygamma/\mygammadot in {0_01/0.01,0_1/0.1,1/1,10/10,100/100}{%
\pgfplotstableread[columns={step_width,\myycolumnname}, col sep=comma]{\mypath/averaged_then_fitted-gamma_\mygammadot.csv}\mybaoabtable

\addplot+[thick,dotted] table[x=step_width, y={create col/linear regression={x=step_width,y=\myycolumnname, variance list={100,10,1,1,1}}}]\mybaoabtable;
\xdef\slopeglaone{\pgfplotstableregressiona}
\addlegendentryexpanded{slope: \pgfmathprintnumber[fixed,precision=2]{\slopeglaone}}

\addplot+[thick,
	no marks,
] table[x=step_width,y=\myycolumnname, col sep=comma]{\mypath/averaged_then_fitted-gamma_\mygammadot.csv};
\expandafter\addlegendentry\expandafter{\mygammadot}

% \addplot+[thick,error bars/.cd, y dir=both, y explicit] table[x=step_width,y expr={abs(0.05-\thisrow{avg_\myycolumnname})/0.05}, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)/0.05}, col sep=comma]{\mypath/estimated-gamma_\mygammadot.csv};
% \expandafter\addlegendentry\expandafter{\mygammadot}
}%
\end{loglogaxis}
\end{tikzpicture}

==> figures/15_Asymptotic_Kinetic_Error/Flat_potential/step_width_asymptotic_error-analytical_solution.tex <==
\def\myN{1e6}%
\def\mybeta{1}%

\begin{tikzpicture}[]
\begin{loglogaxis}[
	width=7cm,height=6cm,
	xlabel = {Step width},
	ylabel = {error},
	grid=major,
	legend pos=outer north east,
	legend columns=1,
	xtick={0.25,0.125,0.0625,0.03125,0.015625},
	log ticks with fixed point,
	cycle list={
		{mark=o,blue},
		blue,
		{mark=square,red},
		red,
		{mark=otimes, brown},
		brown,
		{mark=star,black},
		black,
		{mark=diamond,green},
		green,
	},
	no marks, thick,
]
\foreach \mygamma in {0.01,0.1,1,10,100}{%

\pgfplotstableset{
	create on use/step_width/.style={create col/set list={0.25,0.125,0.0625,0.03125,0.015625}},
	create on use/average_kinetic_error/.style={create col/expr={1/sqrt(1e6*\mybeta)*sqrt((1+exp(-\mygamma*\thisrow{step_width}))/(1-exp(-\mygamma*\thisrow{step_width})))}},
}

\pgfplotstablenew[columns={step_width,average_kinetic_error}]{5}\mytable

%\addplot+[domain={(0.0156:0.25)}] {1/sqrt(\myN)*(1+exp(-\mygamma*x))/(1-exp(-\mygamma*x))};
\addplot table[x=step_width,y=average_kinetic_error]\mytable;
\expandafter\addlegendentry\expandafter{\mygamma}%,\myslope}
\addplot+[dotted] table[x=step_width,y={create col/linear regression={y=average_kinetic_error, variance list={1,1,1,10,100}}}]\mytable;
\xdef\myslope{\pgfplotstableregressiona}
\addlegendentryexpanded{\pgfmathprintnumber[fixed]{\myslope}}
}%
\end{loglogaxis}
\end{tikzpicture}

==> figures/15_Asymptotic_Kinetic_Error/Quadratic_potential/step_width-error_to_asymptotic_value.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Quadratic potential}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/15_Asymptotic_Kinetic_Error/data/Quadratic_potential}\fi%

%special column names
\ifdefined\myxcolumnname\empty\else\def\myxcolumnname{step_width}\fi%
\ifdefined\myycolumnname\empty\else\def\myycolumnname{final_mean_value}\fi%
%parameters
\ifdefined\myfactor\empty\else\def\myfactor{2_}\fi% %0_1,1_,2_
\ifdefined\myfactordot\empty\else\def\myfactordot{2.}\fi% %0.1,1.,2.\ifdefined\mygamma\empty\else\def\mygamma{0.01}\fi% %0.01, 0.1, 1, 10, 100

\begin{tikzpicture}[]
\begin{loglogaxis}[
	%title style={align=left},
	%title = {\emph{\myexperimentname}:\\ dashed - true final value, solid - estimated final value},
	xlabel = {\expandafter\spaceus\expandafter{\myxcolumnname}},
	ylabel = {error to asymptotic value},
	%xtick={0.015625,0.03125,0.0625,0.125,0.25},
	legend pos=outer north east,
	grid=major,
%	each nth point=1,
	cycle multi list={
		black,red,blue,brown,green
	}
]
\addlegendimage{empty legend}
\addlegendentry{\escapeus{gamma}}
\foreach \mygamma in {0.01,0.1,1,10,100}{%
\addplot+[error bars/.cd, y dir=both, y explicit] table[x=\myxcolumnname,y expr={abs(0.05-\thisrow{avg_\myycolumnname})/0.05}, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)/0.05}, col sep=comma]{\mypath/estimated_kinetic_energy-factor_\myfactordot-gamma_\mygamma.csv};
\expandafter\addlegendentry\expandafter{\mygamma}
}%
\end{loglogaxis}
\end{tikzpicture}


==> figures/15_Asymptotic_Kinetic_Error/alpha_values.tex <==
\pgfplotsset{compat=1.5.1}

\pgfplotsset{
logaxisx/.style={
    xmode=log,
    xtick={0.02,0.05,0.2,0.5,2,5,20,50},
    extra x ticks={0.01,0.1,1,10,100},
    minor xtick={0.03,0.04,0.06,0.07,0.08,0.09,0.3,0.4,0.6,0.7,0.8,0.9,3,4,6,7,8,9,30,40,60,70,80,90},
    %xticklabel={\pgfmathfloatparsenumber{\tick}\pgfmathfloatexp{\pgfmathresult}\pgfmathprintnumber{\pgfmathresult}},
    log ticks with fixed point,
    extra x tick style={/pgfplots/major tick length=.2cm,/pgfplots/tick style={line width=1.5pt}},
}
}

\begin{tikzpicture}[]
\begin{axis}[
	width=7cm,height=6cm,
	%title={alpha values},
	xtick={0.25,0.125,0.0625,0.03125,0.015625},
	%log ticks with fixed point,
	xlabel={Step width $\Delta t$},
	ylabel={$\alpha = \exp{(-\gamma \cdot \Delta t)}$},
	xmajorgrids,
	extra x tick style={
		log identify minor tick positions=true},
	legend pos=outer north east,
	xmode=log,
	log ticks with fixed point,
	cycle list={
		{mark=o,blue},{mark=square,red},{mark=otimes, brown},{mark=star,black},{mark=diamond,green}
	},
]
\addlegendentry{$\gamma$}
\addlegendimage{empty legend}
\foreach \mygamma in {0.01,0.1,1,10,100}{%
\addplot+[domain={0.01:0.2}, thick, samples=10] {exp(-(\mygamma)*x)};
\addlegendentryexpanded{\mygamma}
}
\end{axis}
\end{tikzpicture}

==> figures/23_Benchmarking_TFP_vs_TATi_HMC/timing-steps-input_dimension-dimension-output_dimension-batch_size.tex <==
\ifdefined\myexperimentname\empty\else\def\myexperimentname{Tensorflow HMC}\fi%
\ifdefined\mypath\empty\else\def\mypath{\myexperimentspath/23_Benchmarking_TFP_vs_TATi_HMC/data/}\fi%

%special column names
\ifdefined\myxcolumnname\empty\else\def\myxcolumnname{leapfrog_steps}\fi%
\ifdefined\myycolumnname\empty\else\def\myycolumnname{time}\fi%
%parameters
\ifdefined\mysteps\empty\else\def\mysteps{1000}\fi% %1000
\ifdefined\myinputdimension\empty\else\def\myinputdimension{784}\fi% %784
\ifdefined\mydimension\empty\else\def\mydimension{1000}\fi% %1000
\ifdefined\myoutputdimension\empty\else\def\myoutputdimension{10}\fi% %10
\ifdefined\mybatchsize\empty\else\def\mybatchsize{1000}\fi% %550

\begin{tikzpicture}[]
\begin{loglogaxis}[
	title style={align=left},
	title = {\emph{\myexperimentname}:\\ \expandafter\escapeus\expandafter{steps}=\pgfmathprintnumber{\mysteps}, \expandafter\escapeus\expandafter{input_dimension}=\pgfmathprintnumber{\myinputdimension}, \expandafter\escapeus\expandafter{dimension}=\pgfmathprintnumber{\mydimension},\\ \expandafter\escapeus\expandafter{output_dimension}=\pgfmathprintnumber{\myoutputdimension}, \expandafter\escapeus\expandafter{batch_size}=\pgfmathprintnumber{\mybatchsize}},
	xlabel = {\expandafter\spaceus\expandafter{\myxcolumnname}},
	ylabel = {\expandafter\spaceus\expandafter{\myycolumnname}},
	xtick={1,10,5,50},
	legend pos=outer north east,
	%cycle list name=exotic,
	grid=major,
%	each nth point=1,
]
\addplot+[error bars/.cd, y dir=both, y explicit] table[x=\myxcolumnname,y=avg_\myycolumnname, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)}, col sep=comma]{\mypath/Tensorflow_HMC/timing-batch_size_\mybatchsize-dimension_\mydimension-input_dimension_\myinputdimension-output_dimension_\myoutputdimension-steps_\mysteps.csv};
\addlegendentry{TFP}

\addplot+[error bars/.cd, y dir=both, y explicit] table[x=\myxcolumnname,y=avg_\myycolumnname, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)}, col sep=comma]{\mypath/Tensorflow_HMC_placeholders/timing-batch_size_\mybatchsize-dimension_\mydimension-input_dimension_\myinputdimension-output_dimension_\myoutputdimension-steps_\mysteps.csv};
\addlegendentry{TFP placeholders}

\addplot+[error bars/.cd, y dir=both, y explicit] table[x=\myxcolumnname,y=avg_\myycolumnname, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)}, col sep=comma]{\mypath/TATiSampler_HMC_2ndOrder/timing-batch_size_\mybatchsize-dimension_\mydimension-input_dimension_\myinputdimension-output_dimension_\myoutputdimension-steps_\mysteps.csv};
\addlegendentry{TATiSampler}

%\addplot+[error bars/.cd, y dir=both, y explicit] table[x=\myxcolumnname,y=avg_\myycolumnname, y error expr={sqrt(\thisrow{var_\myycolumnname}-\thisrow{avg_\myycolumnname}^2)}, col sep=comma]{\mypath/TATi_simulation_HMC_2ndOrder/timing-batch_size_\mybatchsize-dimension_\mydimension-input_dimension_\myinputdimension-output_dimension_\myoutputdimension-steps_\mysteps.csv};
%\addlegendentry{TATi.simulation}
\end{loglogaxis}
\end{tikzpicture}


==> figures/TATi/computational_graph.tex <==
\usetikzlibrary{arrows,positioning}
\tikzset{%
 % >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
	base/.style = {circle,draw=black, minimum width=1cm,minimum height=1cm,
		text centered, font=\Large\sffamily},
	tensorflow_node/.style = {base, pattern=bricks, pattern color=gray!70},
	variable_node/.style = {base, pattern=north east lines, pattern color=gray!70},
	placeholder_node/.style = {base, pattern=crosshatch dots, pattern color=gray!70},
pil/.style={
           ->,
           very thick,
           shorten <=3pt,
           shorten >=3pt,}
}

\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]

\node (rate)	[placeholder_node]	{$\Delta t$};
\node (scaled_grad)	[tensorflow_node,below of=rate]	{$\prod$};
\node (grad)	[variable_node, left of=scaled_grad]	{$\nabla L(\theta)$};
\node (pos)	[variable_node,below of=scaled_grad]	{$\theta$};
\node (sum)	[tensorflow_node,right of=scaled_grad,yshift=-.8cm,]	{$\Sigma$};
\node (assign)	[tensorflow_node,right of=sum]	{$\rightarrow$};

\draw[pil] (scaled_grad) -- (sum);
\draw[pil] (grad) -- (scaled_grad);
\draw[pil] (rate) -- (scaled_grad);
\draw[pil] (pos) -- (sum);
\draw[pil] (sum) -- (assign);
\draw[pil] (assign) edge[bend left] (pos);

\end{tikzpicture}


==> figures/TATi/tati-architecture.tex <==
\usetikzlibrary{positioning,backgrounds,fit}

\tikzset{%
 % >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
            base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1cm,
                           text centered, font=\sffamily},
	tensorflow/.style = {base, pattern=crosshatch dots, pattern color=blue!60},
	tati/.style = {base, pattern=crosshatch dots, pattern color=red!60},
	tati_highlevel/.style = {base, pattern=crosshatch dots, pattern color=red!60},
	user/.style = {base,fill=green!30},
%          process/.style = {base, minimum width=2.5cm, fill=orange!15,
%                            font=\ttfamily},
}

\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]

% base
\node (tf_data_Dataset)	[tensorflow]	{TF Dataset};
\node (tf_optimizer)			[tensorflow, right of=tf_data_Dataset, xshift=2.6cm]		{TF Optimizer};
\node (tf_core)				[tensorflow, right of=tf_optimizer, xshift=2.5cm]	{TF Core};

% tati
\node (tati_inputpipeline)			[tati, above of=tf_data_Dataset, xshift=-.5cm]	{TATi Input Pipeline};
\node (tf_sampler)			[tensorflow, above of=tf_optimizer]	{TF Sampler};
\node (tati_walkers)			[tati, above of=tf_core, text width=3.4cm]	{Ensemble of Walkers};

% tati interface
\node (tati_models)			[tati_highlevel, above of=tf_sampler, text width=10.77cm,xshift=0.6cm]	{TATi modules};

% tools
\node (tati_optimizer)		[tati_highlevel, above of=tati_models, minimum width=2.5cm, xshift=-4.5cm,yshift=.5cm]	{TATi \\ Optimizer};
\node (tati_sampler)		[tati_highlevel, above of=tati_optimizer, minimum width=2.5cm]	{TATi \\ Sampler};
\node (tati_explorer)		[tati_highlevel, above of=tati_sampler, minimum width=2.5cm]	{TATi \\ Explorer};

\node (tati_inputspacesampler)		[tati_highlevel, right of=tati_optimizer, minimum width=2.5cm, xshift=1.5cm]	{TATi \\ InputSpace \\ Sampler};
\node (tati_lossfunctionsampler)		[tati_highlevel, above of=tati_inputspacesampler, minimum width=2.5cm, xshift=.2cm]	{TATi \\ LossFunction \\ Sampler};

\node (tati_analyser)		[tati_highlevel, above of=tati_lossfunctionsampler, minimum width=2.5cm, minimum height=1.4cm]	{TATi \\ Analyser};

% user
\node (tati_simulation)			[tati_highlevel, right of=tati_inputspacesampler, text width=2cm, xshift=2.5cm]	{TATi simulation interface};

\node (_)			[ right of=tati_analyser, fill=green!20, xshift=2cm, yshift=.6cm] {};

%% connections
%\draw[] (tf_data_Dataset) -- (tf_data_Dataset.north|-tati_inputpipeline.south);
%\draw[] (tf_optimizer) -- (tf_optimizer.north|-tf_sampler.south);
%\draw[] (tf_core) -- (tf_core.north|-tati_walkers.south);

%% grouping boxes
\begin{scope}[on background layer]
	\node [fit=(tf_core) (tf_data_Dataset),inner sep=4mm,fill=cyan!15] (tensorflow)
	{\vspace{3em}Tensorflow};
	
	\node [fit=(tf_sampler) (tati_inputpipeline) (tati_walkers) (tati_models),inner sep=4mm,fill=red!20] (tati_module)
	{\vspace{0.5em}Thermodynamic Analytics Toolkit};
	
	\node [fit=(tati_optimizer) (tati_sampler) (tati_explorer)(tati_inputspacesampler) (tati_lossfunctionsampler) (tati_analyser) ,inner sep=6mm,fill=green!20] (generation)
	{\vspace{3.5em}TATi tools};

	\node [fit=(tati_simulation) (_),inner sep=6mm,fill=green!20] (user_space)
	{User sampling codes};

	\draw[] (generation) -- (generation.south|-tati_module.north);
	%\draw[] (analysis) -- (analysis.south|-tati_module.north);
	\draw[] (user_space) -- (user_space.south|-tati_module.north);
	\draw[] (tensorflow) -- (tensorflow|-tati_module.south);
\end{scope}

\end{tikzpicture}


==> figures/TATi/tati-mindmap.tex <==
\begin{tikzpicture}[ every annotation/.style = {draw,
                     fill = white, font = \Large},
	tools/.style={sibling angle=40,level distance=12em},
	samplers/.style={level distance=11em},
	methods/.style={sibling angle=40,level distance=12em},
	simulations/.style={sibling angle=30},
]

\path[mindmap,concept color=black!40,text=white,
    every node/.style={concept,},%circular drop shadow},
    root/.style    = {concept color=black!40,
      font=\Large\bfseries,text width=10em},
    level 1 concept/.append style={font=\Large\bfseries,
		sibling angle=90,
		text width=7.7em,
    level distance=17em,inner sep=10pt},
    level 2 concept/.append style={font=\bfseries,inner sep=0pt,level distance=11em},
  ]
	node [font=\Large\bfseries] (tati) {Thermodynamic \\ Analytics \\ Toolkit} [clockwise from=0]
	child[concept color=gray!60] {
		node[] {\hspace{-2em}Samplers} [clockwise from=130] {
			child [samplers]{ node[] {BAOAB} }
			child [samplers]{ node[] {GLA1} }
			child [samplers]{ node[] {GLA2} }
			child [samplers]{ node[] {SGLD} }
			child [samplers]{ node[] {HMC} }
		}
	}
	child[sibling angle=90,level distance=20em,concept color=gray!60] {
		node {\hspace{-2em}Simulations \\ \hspace{-2em}Interface} [clockwise from=30] 
		{
			child [simulations]{ node[] {loss()} }
			child [simulations]{ node[] {gradient()} }
			child [simulations]{ node[] {hessian()} }
			child [simulations]{ node[] {para- \\ meters} }
			child [simulations]{ node[] {momenta} }
			child [simulations]{ node[] {averages} }
			child [simulations]{ node[] {fit()} }
			child [simulations]{ node[] {score()} }
			child [simulations]{ node[] {predict()} }
		}
	}
	child[pattern=north west lines] {
		node {\hspace{-2em}Enhanced \\ \hspace{-2em}Sampling \\ \hspace{-2em}Methods} [clockwise from=240]  {
			child [level distance=13em] { node [text width=2.4cm] {Ensemble of Walkers} }
			child [level distance=13em] { node [text width=2.4cm] {Covariance-Controlling \\ Thermostats} }
			child [level distance=13em] { node [text width=2.4cm] {Diffusion \\ Maps} }
		}
	}
	child [concept color=black!60] {
		node {\hspace{-2em}Tools} [clockwise from=190]  {
			child [tools]{ node[text width=2.4cm] {TATi\-Optimizer} }
			child [tools]{ node[text width=2.4cm] {TATi\-Sampler} }
			child [tools]{ node[text width=2.4cm] {TATi\-Explorer} }
			child [tools]{ node[text width=2.4cm] {TATi\-LossFunction\-Sampler} }
			child [tools]{ node[text width=2.4cm] {TATi\-InputSpace\-Sampler} }
			child [tools]{ node[text width=2.4cm] {TATi\-Analyser} }
		}
	};

\end{tikzpicture}


==> figures/TATi/tati_simulations-architecture.tex <==
\usetikzlibrary{backgrounds,fit}

\tikzset{%
 % >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
            base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1cm,
                           text centered, font=\sffamily},
	tensorflow/.style = {base, pattern=north east lines, pattern color=gray!60},
	tati/.style = {base, pattern=north west lines, pattern color=gray!60},
	tati_highlevel/.style = {base, pattern=crosshatch dots, pattern color=gray!60},
	pydiffmap/.style = {base},
	user/.style = {base,fill=gray!30},
%          process/.style = {base, minimum width=2.5cm, fill=orange!15,
%                            font=\ttfamily},
}

\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]

% base
\node (tf_data_Dataset)	[tensorflow]	{TF Dataset};
\node (tf_optimizer)			[tensorflow, right of=tf_data_Dataset, xshift=2cm]		{TF Optimizer};
\node (tf_core)				[tensorflow, right of=tf_optimizer, xshift=2.5cm]	{TF Core};

% tati
\node (tati_inputpipeline)			[tati, above of=tf_data_Dataset]	{TATi Input Pipeline};
\node (tf_sampler)			[tati, above of=tf_optimizer]	{TF Samplers};
\node (tati_walkers)			[tati, above of=tf_core, text width=3.4cm]	{Ensemble of Walkers};

% simulations
\node (tati_simulations)			[tati_highlevel, above of=tf_sampler, text width=10.77cm,xshift=0.6cm]	{TATi modules: simulation, model, analysis};

% user
\node (user)			[user, above of=tati_simulations, text width=10.77cm]	{User sampling codes};

%% connections
\draw[] (tati_walkers) -- (tati_walkers.north|-tati_walkers.south);

\draw[] (tf_sampler) -- (tf_sampler.north|-tati_simulations.south);
\draw[] (tati_inputpipeline) -- (tati_inputpipeline.north|-tati_simulations.south);
\draw[] (tati_walkers) -- (tati_walkers.north|-tati_simulations.south);

%% grouping boxes
\begin{scope}[on background layer]
 \node[fit=(tf_core) (tf_data_Dataset),inner sep=3mm,fill=gray!15] (tensorflow){\vspace{3.05em}Tensorflow};
 \node[fit=(tf_sampler) (tati_inputpipeline) (tati_walkers) (tati_simulations),inner sep=3mm,fill=gray!20] (tati){\vspace{8.4em}Thermodynamic Analytics Toolkit};

\draw[] (tensorflow) -- (tensorflow|-tati.south);
\draw[] (tati) -- (tati|-user.south);
\end{scope}

\end{tikzpicture}


==> figures/TATi/tati_tools-architecture.tex <==
\usetikzlibrary{positioning,backgrounds,fit}

\tikzset{%
 % >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
            base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1cm,
                           text centered, font=\sffamily},
	tensorflow/.style = {base, pattern=north east lines, pattern color=gray!60},
	tati/.style = {base, pattern=north west lines, pattern color=gray!60},
	tati_highlevel/.style = {base, pattern=crosshatch dots, pattern color=gray!60},
%          process/.style = {base, minimum width=2.5cm, fill=orange!15,
%                            font=\ttfamily},
}

\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]

% base
\node (tf_data_Dataset)	[tensorflow]	{TF Dataset};
\node (tf_optimizer)			[tensorflow, right of=tf_data_Dataset, xshift=2.6cm]		{TF Optimizer};
\node (tf_core)				[tensorflow, right of=tf_optimizer, xshift=2.5cm]	{TF Core};

% tati
\node (tati_inputpipeline)			[tati, above of=tf_data_Dataset, xshift=-.5cm]	{TATi Input Pipeline};
\node (tf_sampler)			[tati, above of=tf_optimizer]	{TF Sampler};
\node (tati_walkers)			[tati, above of=tf_core, text width=3.4cm]	{Ensemble of Walkers};

% tools
\node (tati_optimizer)		[tati_highlevel, above of=tati_inputpipeline, minimum width=1.5cm, xshift=-.5cm,yshift=.5cm]	{TATi \\ Optimizer};
\node (tati_sampler)		[tati_highlevel, right of=tati_optimizer, minimum width=1.5cm]	{TATi \\ Sampler};
\node (tati_explorer)		[tati_highlevel, right of=tati_sampler, minimum width=1.5cm]	{TATi \\ Explorer};

\node (tati_inputspacesampler)		[tati_highlevel, right of=tati_explorer, minimum width=1.5cm, xshift=1cm]	{TATi \\ InputSpace \\ Sampler};
\node (tati_lossfunctionsampler)		[tati_highlevel, right of=tati_inputspacesampler, minimum width=1.5cm, xshift=.2cm]	{TATi \\ LossFunction \\ Sampler};

\node (tati_analyser)		[tati_highlevel, right of=tati_lossfunctionsampler, minimum width=1.5cm, minimum height=1.4cm]	{TATi \\ Analyser};

%% connections
%\draw[] (tf_data_Dataset) -- (tf_data_Dataset.north|-tati_inputpipeline.south);
%\draw[] (tf_optimizer) -- (tf_optimizer.north|-tf_sampler.south);
%\draw[] (tf_core) -- (tf_core.north|-tati_walkers.south);

%% grouping boxes
\begin{scope}[on background layer]
	\node [fit=(tf_core) (tf_data_Dataset),inner sep=4mm,fill=gray!15] (tensorflow){\vspace{3em}Tensorflow};
	\node [fit=(tf_sampler) (tati_inputpipeline) (tati_walkers) ,inner sep=4mm,fill=gray!20] (tati_module){\vspace{3.5em}Thermodynamic Analytics Toolkit};
	\node [fit=(tati_optimizer) (tati_sampler) (tati_explorer) ,inner sep=6mm,fill=gray!30] (generation){\vspace{3.5em}Generate Trajectories};
	\node [fit=(tati_inputspacesampler) (tati_lossfunctionsampler) (tati_analyser) ,inner sep=4mm,fill=gray!30] (analysis){\vspace{4.5em}Analyse and Visualize};

	\draw[] (generation) -- (generation.south|-tati_module.north);
	\draw[] (analysis) -- (analysis.south|-tati_module.north);
	\draw[] (tensorflow) -- (tensorflow|-tati_module.south);
\end{scope}

\end{tikzpicture}

